Understanding Stress, Burnout, and Behavioral Patterns in Medical Residents Using Large-scale Longitudinal Wearable Recordings

Medical residency training is often associated with physically intense and emotionally demanding tasks, requiring them to engage in extended working hours providing complex clinical care. Residents are hence susceptible to negative psychological effects, including stress and anxiety, that can lead to decreased well-being, affecting them achieving desired training outcomes. Understanding the daily behavioral patterns of residents can guide the researchers to identify the source of stress in residency training, offering unique opportunities to improve residency programs. In this study, we investigate the workplace behavioral patterns of 43 medical residents across different stages of their training, using longitudinal wearable recordings collected over a 3-week rotation. Specifically, we explore their ambulatory patterns, the computer access, and the interactions with mentors of residents. Our analysis reveals that residents showed distinct working behaviors in walking movement patterns and computer usage compared to different years in the program. Moreover, we identify that interaction patterns with mentoring doctors indicate stress, burnout, and job satisfaction.

==> tmp.tex <==

there is a need to investigate working behavior to identify the source of negative impact factors associated with nursing professions.  We investigate workplace behaviors using unobtrusively obtained longitudinal multimodal sensor data in a real-world hospital setting. 


 can cause a significant degree of burnout, leading to interference with individuals' ability to establish rapport, sort through diagnostic dilemmas, and work though complex treatment decision making.


Significantly, the educational phase of residency is linked with demanding and intersecting pressures that encompass cognitive, physical, emotional, and social aspects. For instance, the standard practice in residency training involves medical residents engaging in 12-hour daily commitments. Beyond the extended work hours, the learning experience during residency is emotionally taxing, necessitating medical residents to deliver compassionate and empathetic care while maintaining professionalism. Moreover, medical residents frequently confront evolving and challenging situations, such as the recent global occurrences like the COVID-19 outbreaks, which have presented unparalleled challenges to healthcare systems worldwide \cite{remuzzi2020covid}.


In addition to the physical demands, nursing is also emotionally demanding, requiring the delivery of humane, empathetic, and culturally sensitive care over extended periods \cite{cricco2014need}.
Consequently, they are particularly susceptible to stress, anxiety, and other negative psychological effects that can lead to burnout, job dissatisfaction, and depression \cite{iacovides2003relationship, glass1993depression}.


, which is crucial in preparing medical students with real clinical experiences, often brings unprecedented challenges and significant work demands to medical residents.

Workplace wellness is ever more important, especially in navigating the ever-increasing and competing cognitive, physical, and social demands.

frequently deal with intense and competing demands that are cognitive, physical, emotional, and social in their day-to-day training. Increasingly, they often encounter challenging and emerging circumstances in nature, such as the COVID-19 outbreaks in the last few years that are placing an unprecedented challenge to healthcare systems worldwide \cite{remuzzi2020covid}. 

Notably, nursing, which is at the core of the modern healthcare system, is facing unprecedented challenges and significant increases in work demand. Nursing is known to be stressful: they are required to work long shifts, typically $12$ hours in duration \cite{richardson_12hour, dabner_12hour}.

Workplace wellness is ever more important, especially in navigating the ever-increasing and competing cognitive, physical, and social demands. Emerging crises such as the COVID-19 pandemic have underscored the importance of investigating ways of supporting the well-being of workers, especially in high-stakes domains such as healthcare. 
%brought enormous attention to the research field to investigate ways to support the healthcare system. 
Notably, nursing, which is at the core of the modern healthcare system, is facing unprecedented challenges and significant increases in work demand. Nursing is known to be stressful: they are required to work long shifts, typically $12$ hours in duration \cite{richardson_12hour, dabner_12hour}. Increasingly nurses have to handle the intense workload while providing in-patient nursing care that requires constant vigilance and meticulousness. In addition to the physical demands, nursing is also emotionally demanding, requiring the delivery of humane, empathetic, and culturally sensitive care over extended periods \cite{cricco2014need}.
Consequently, they are particularly susceptible to stress, anxiety, and other negative psychological effects that can lead to burnout, job dissatisfaction, and depression 

frequently deal with challenging and emerging circumstances, such as the COVID-19 outbreaks in the last few years that are placing an unprecedented challenge to healthcare systems worldwide \cite{remuzzi2020covid},

that stress and burnout have widely existed in residency learning, not only increasing the implications for patient care while at residency but also decreasing the health and well-being of medical residents. 

managing competing demands that are cognitive, physical, psychological and social in nature.


Burnout in health care professionals has gained significant attention over the last several years. Given the intense emotional demands of the work environment, clinicians are particularly susceptible to developing burnout above and beyond usual workplace stress. Residency training, in particular, can cause a significant degree of burnout, leading to interference with individuals' ability to establish rapport, sort through diagnostic dilemmas, and work though complex treatment decision making. Overall, burnout is associated with a variety of negative consequences including depression, risk of medical errors, and negative effects on patient safety. The goal of this review is to provide medical educators and leaders with an overview of the existing factors that contribute to burnout, the impact of burnout, interspecialty variation, and suggestions for interventions to decrease burnout.

Nursing professionals as direct clinical providers play a central role in the frontlines of the healthcare system, managing competing demands that are cognitive, physical, psychological and social in nature. They frequently deal with novel and emerging circumstances, such as the ongoing COVID-19 outbreaks that are placing an unprecedented challenge to healthcare systems worldwide \cite{remuzzi2020covid}, and pose a significant increase in the demand for care services. Nurses typically work shifts in long hours ($8$-$12$ hours), with few breaks for rest and meals \cite{stimpfel2012longer}. The prolonged working hours combined with a high-intensity workload can have acute adverse health effects for nurses, which lead to burnout and job dissatisfaction \cite{park2005multilevel, kunaviktikul2015nurses}.




The global understanding is that stress and burnout among resident physicians not only have implications for patient care but also affect the health and well-being of our professional community, emphasizing the importance of well-prepared doctors in providing high-quality and safe patient care through residency training [1].

 Worldwide, medical educationalists and clinicians involved in residency training are focused on the improvement of education through modernizations including implementing competency based learning and assessing and advancing the quality of residents' education through 


Stress and burnout among residency learning 


Medical residency programs take place after training has been completed at an Allopathic or Osteopathic Medical school and offer in-depth, practical training in a chosen medical specialty.


gained significant attention over the last several years. Given the intense emotional demands of the work environment, clinicians are particularly susceptible to developing burnout above and beyond usual workplace stress. 




It is globally understood that high quality and safe patient care can only be provided if doctors are well prepared for this task through (residency) training [1]. Worldwide, medical educationalists and clinicians involved in residency training are focused on the improvement of education through modernizations including implementing competency based learning and assessing and advancing the quality of residents' education through accreditation standards [2, 3]. Ultimately, societies need to know if it matters how, where and by whom doctors were trained.

Stress and burnout among resident physicians have implications for patient care and the health and well-being of our professional community. Sources of such stress in resident training can be divided into three components: 1) situational (workload, sleep deprivation, and poor learning environment); 2) personal (family, isolation, and finan-cial);  and 3) professional (overwhelming patient responsibility and information).1–3Stress resulting from the discrepancy between the individual’s ideals or expectations and the reality of occupational life is a source of burnout.4 Burnout is a “syndrome of emotional exhaustion, depersonalization, and reduced personal accomplishment”,5and can lead to negative repercussions for the individual experiencing burnout, the 

% Contrary to these previous studies, we propose using wearable sensors to provide quantitative measurements of the behavioral patterns of medical residents.

It is worth noting that these behavioral variables have been shown to correlate with workplace stress and burnout in other occupations.


\begin{itemize}[leftmargin=*]
    \item Are behavioral patterns of residents different in their training experiences?

    \vspace{0.5mm}

    \item Would there be unique behavioral patterns of residents at different times in their training shift?
    
    \vspace{0.5mm}
    
    \item Are behavioral patterns indicative of stress, burnout, and anxiety?
    
    
\end{itemize}

    % \item\textbf{Anxiety} We evaluated anxiety of residents through State-Trait Anxiety Inventory (STAI) \cite{Spielberger.STAI.1983}, consisting 20 items on a four-point scale. The final STAI was scored by summing responses, resulting in a value in the range 20 to 80, with higher scores indicating greater anxiety.

    
% As we focus on studying stress associated with residents, we include EMA responses related to stress, job performance, and work context, as described below. 



% From the two-sample independent t-test results shown in Table \ref{tab:demographics_igtb}, the day shift group and night shift group do not differ in the STAI scores, the PANAS scores, or the personality. However, the day shift group and night shift group differ significantly in reported life satisfaction scores (day shift: $14.9\pm3.7$; night shift nurses: $16.5\pm4.9$; $t(111) = 2.21, p = 0.030$). From the three-way ANOVA tests, the shift schedule ($F(1, 108) = 3.99, p = 0.048$) is significant for the SWLS, but gender and age do not have an effect on SWLS. Additionally, night shift nurses report significantly higher PSQI scores than day shift nurses, indicating poor sleep quality (day shift: $7.0\pm2.0$; night shift nurses: $8.4\pm2.5$; $t(110) = -2.97, p = 0.004$). Similarly, age and gender are not significant for PSQI scores from the ANOVA analysis, but the shift was ($F(1, 108) = 4.40, p = 0.038$). Although shift type is not significant for openness from the independent t-test, the three-way ANOVA analysis shows that the primary shift schedule ($F(1, 107) = 7.65, p = 0.007$) is significant for the openness with the covariates as age and gender.

% The analysis in this work included $n=43$ residents with a minimum of 3 days of Fitbit recordings, of which $n=28$ ($65\%$) were male, and $n=15$ ($35\%$) were female, as shown in Figure~\ref{fig:demographics}. Most participants enrolled in the Internal Medicine program ($n=36$, $84\%$), and the remaining residents were in the Emergency Medicine program ($n=7$, $16\%$). The year in the program ranges from $1$ to $3$, with $n=16$ participants as resident interns (first year), $n=15$ participants as junior residents, and $n=12$ participants as senior residents.


% The residents normally take notes and plan lab orders after the morning round till noon. and the amount of teaching during each patient visit

        \multicolumn{1}{l}{\hspace{0.25cm}{Rest-activity}} &
        \multicolumn{1}{c}{$30.5$ ($11.6$)} &
        \multicolumn{1}{c}{$24.8$ ($14.1$)} &
        \multicolumn{1}{c}{0.187}  \rule{0pt}{2.25ex} \\



        \multicolumn{1}{l}{\hspace{0.15cm}{Fellow Dr. Interaction}} &
        \multicolumn{1}{c}{$79.0$ ($21.4$)} &
        \multicolumn{1}{c}{$84.8$ ($23.6$)} &
        \multicolumn{1}{c}{0.461}  \rule{0pt}{2.25ex} \\

        \multicolumn{1}{l}{\hspace{0.15cm}{Attending Dr. Interaction}} &
        \multicolumn{1}{c}{$65.6$ ($27.5$)} &
        \multicolumn{1}{c}{$73.1$ ($25.8$)} &
        \multicolumn{1}{c}{0.477}  \rule{0pt}{2.25ex} \\
                    

\subsection{Ecological Momentary Assessments (EMAs)}
    
In addition to pre-study surveys, the EMAs were administered twice daily throughout the study period. The midday EMA is a one-item survey evaluating stress, and the \emph{end-of-day EMA} assesses daily stressors, work behaviors, and sleep. Given the scope of this study, we include EMAs related to stress, job performance, and work context.

% \item\textbf{Depression} 
    % Depression was evaluated using the \emph{Patient Health Questionnaire} (PHQ-9) \cite{Kroenke.JGIM.2001}. Participants rated 9 items about depressive symptoms in the past two weeks on a scale from 0 to 3, with higher scores indicating greater depression. The final score is obtained by summing items.


        \cmidrule(lr){1-4}

        \textbf{Midday EMA} & Stress & - & 1-7 ($\uparrow$) \\

        \cmidrule(lr){1-4}
        \multirow{2}{*}{\textbf{End-of-day EMA}} & Stress & - & 1-7 ($\uparrow$) \\

        & Work Context & - & - \\

        % & Job Performance & - & 1-6 ($\uparrow$) \\

% In this study, we deploy two survey types to evaluate the behavioral variables of residents: a one-time assessment prior to the start of the study and ecological momentary assessments throughout the study. We summarize the surveys, behavioral variables, and scoring scales in this work in Tabel~\ref{tab:self_report}


% explore the behavioral patterns of residents, especially those related to daily training, to identify the source of stress and burnout associated with residency training.

% For example, the standard practice in residency training involves residents engaging in a prolonged working routine (typically $>10$ hours) and complex working procedures involving problem solving and decision making.


% Last but not least, medical residents frequently encounter uniquely challenging and emerging circumstances, such as the recent COVID-19 outbreaks, which have presented unprecedented challenges to healthcare systems worldwide \cite{remuzzi2020covid}. 


% As a result, residents are particularly susceptible to stress, anxiety, and other adverse psychological effects, making them more vulnerable to developing burnout \cite{ishak2009burnout, prins2007burnout}. If not properly managed, challenges to stress and burnout may contribute to declines in the health and well-being of residents, increasing the implications in delivering patient care. Furthermore, these unwanted impacts can lead to negative training outcomes, interfering with residents to establish the ability to make informed decisions and plans in patient monitoring, medical treatment, and clinical rehabilitation. Therefore, it is critical for researchers to investigate the behavioral patterns of residents, especially those related to daily training, to identify the source of stress and burnout associated with residency training.
.

% \subsection{Pre-study Assessment}

\begin{itemize}[leftmargin=*]
    \item\textbf{Midday EMA} asked residents about stress in the morning on a 7-scale, with higher scores indicating higher stress.
    \vspace{0.5mm}
    
    \item\textbf{End-of-day EMA} instructed participants to report their stress during the afternoon on a scale from not at all stressed (1) to a great deal of stress (7). Moreover, participants were asked whether they were in the hospital that day. 

\end{itemize}


\begin{itemize}[leftmargin=*]
    \item\textbf{Midday EMA} asked residents about stress in the morning on a 7-scale, with higher scores indicating higher stress.
    \vspace{0.5mm}
    
    \item\textbf{End-of-day EMA} \hspace*{1em}
        \begin{itemize}
            \item\textbf{Stress} Similar to midday EMA, participants reported their stress levels during the afternoon on a scale from not at all stressed (1) to a great deal of stress (7).
            \vspace{0.5mm}

            \item\textbf{Work Context} Participants were asked to respond whether they were in the hospital or not that day. 
            
            \vspace{0.5mm}

            % \item\textbf{Job Performance} This EMAs also asked participants to rate perceived job performance on a 6-point scale, with higher scores indicating greater job performance.
            
            \vspace{0.5mm}

        \end{itemize}

\end{itemize}

We plot the average scales of pre-study evaluation and daily EMAs to the year in the program (intern; junior/senior) as demonstrated in Figure~\ref{fig:surveys}. We perform two-sample independent t-test results on the self-report assessment variables conditioned on the year in the program. 

\noindent \textbf{Pre-study Assessment} The t-test shows that residents do not differ in the PSS, OBI, and STAI scores to the year in the program. Moreover, as we instructed the same survey to evaluate the anxiety levels of nursing professionals in \cite{feng2021multimodal}, we compare the STAI scores of residents with day and night shift nurses, revealing that residents have significantly higher anxiety scores than nurses (Residents: $42.10\pm5.21$; Day-shift Nurse: $32.88\pm7.63$; Day-shift Nurse: $35.43\pm9.08$; $p<0.01$). This result implies that residents experience greater anxiety impacts than other healthcare providers.

\noindent \textbf{EMAs} The t-test shows that resident interns and juniors/seniors do not differ in the midday and end-of-day (eod) stress scores. However, we observe that resident interns have higher levels of stress than junior/senior interns on average in Fig~\ref{fig:surveys}.

% Moreover, as we instructed the same survey to evaluate the anxiety levels of nurses, we compare the STAI scores of residents with day and night shift nursing staff in \cite{feng2021multimodal}, revealing that residents have significantly higher anxiety scores than nurses (Residents: $42.10\pm5.21$; Day-shift Nurse: $32.88\pm7.63$; Day-shift Nurse: $35.43\pm9.08$; $p<0.01$). This result implies that residents experience greater negative mental impacts than other healthcare providers.






